dup -- Explicit un-sharing in Haskell

We propose two operations to prevent sharing in Haskell that do not require modifying the data generating code, demonstrate their use and usefulness, and compare them to other approaches to preventing sharing. Our claims are supported by a formal semantics and a prototype implementation.

==> statstable-slow.tex <==
\makeatletter
\begin{tabular}{lrrrrrrrrrrrr}
 \\
& \multicolumn{2}{c}{no sharing}& \multicolumn{2}{c}{shared tree}& \multicolumn{2}{c}{add. thunk}& \multicolumn{2}{c}{partly eval'ed}& \multicolumn{2}{c}{fully eval'ed}& \multicolumn{2}{c}{run twice} \\
& MB & sec.& MB & sec.& MB & sec.& MB & sec.& MB & sec.& MB & sec. \\ \midrule 
original%
&
 {\def\@currentlabel{2}\label{stats:slow:Original:Unshared:mem}2} &
 {\def\@currentlabel{108.70}\label{stats:slow:Original:Unshared:time}108.70}&
 {\def\@currentlabel{1\,641}\label{stats:slow:Original:Shared:mem}1\,641} &
 {\def\@currentlabel{115.72}\label{stats:slow:Original:Shared:time}115.72}&
 {\def\@currentlabel{1\,643}\label{stats:slow:Original:SharedThunk:mem}1\,643} &
 {\def\@currentlabel{113.99}\label{stats:slow:Original:SharedThunk:time}113.99}&
 {\def\@currentlabel{1\,642}\label{stats:slow:Original:SharedEvaled:mem}1\,642} &
 {\def\@currentlabel{115.47}\label{stats:slow:Original:SharedEvaled:time}115.47}&
 {\def\@currentlabel{1\,641}\label{stats:slow:Original:SharedFull:mem}1\,641} &
 {\def\@currentlabel{119.01}\label{stats:slow:Original:SharedFull:time}119.01}&
 {\def\@currentlabel{1\,641}\label{stats:slow:Original:RunTwice:mem}1\,641} &
 {\def\@currentlabel{118.89}\label{stats:slow:Original:RunTwice:time}118.89} \\
\textsf{solveDup}%
&
 {\def\@currentlabel{2}\label{stats:slow:SolveDup:Unshared:mem}2} &
 {\def\@currentlabel{108.76}\label{stats:slow:SolveDup:Unshared:time}108.76}&
 {\def\@currentlabel{2}\label{stats:slow:SolveDup:Shared:mem}2} &
 {\def\@currentlabel{108.71}\label{stats:slow:SolveDup:Shared:time}108.71}&
 {\def\@currentlabel{1\,643}\label{stats:slow:SolveDup:SharedThunk:mem}1\,643} &
 {\def\@currentlabel{114.19}\label{stats:slow:SolveDup:SharedThunk:time}114.19}&
 {\def\@currentlabel{1\,642}\label{stats:slow:SolveDup:SharedEvaled:mem}1\,642} &
 {\def\@currentlabel{115.63}\label{stats:slow:SolveDup:SharedEvaled:time}115.63}&
 {\def\@currentlabel{1\,641}\label{stats:slow:SolveDup:SharedFull:mem}1\,641} &
 {\def\@currentlabel{118.96}\label{stats:slow:SolveDup:SharedFull:time}118.96}&
 {\def\@currentlabel{2}\label{stats:slow:SolveDup:RunTwice:mem}2} &
 {\def\@currentlabel{217.26}\label{stats:slow:SolveDup:RunTwice:time}217.26} \\
\textsf{rateDup}%
&
 {\def\@currentlabel{2}\label{stats:slow:RateDup:Unshared:mem}2} &
 {\def\@currentlabel{141.53}\label{stats:slow:RateDup:Unshared:time}141.53}&
 {\def\@currentlabel{8}\label{stats:slow:RateDup:Shared:mem}8} &
 {\def\@currentlabel{141.92}\label{stats:slow:RateDup:Shared:time}141.92}&
 {\def\@currentlabel{9}\label{stats:slow:RateDup:SharedThunk:mem}9} &
 {\def\@currentlabel{139.00}\label{stats:slow:RateDup:SharedThunk:time}139.00}&
 {\def\@currentlabel{9}\label{stats:slow:RateDup:SharedEvaled:mem}9} &
 {\def\@currentlabel{141.82}\label{stats:slow:RateDup:SharedEvaled:time}141.82}&
 {\def\@currentlabel{1\,641}\label{stats:slow:RateDup:SharedFull:mem}1\,641} &
 {\def\@currentlabel{119.35}\label{stats:slow:RateDup:SharedFull:time}119.35}&
 {\def\@currentlabel{1\,638}\label{stats:slow:RateDup:RunTwice:mem}1\,638} &
 {\def\@currentlabel{258.22}\label{stats:slow:RateDup:RunTwice:time}258.22} \\
\textsf{solveDeepDup}%
&
 {\def\@currentlabel{2}\label{stats:slow:SolveDeepDup:Unshared:mem}2} &
 {\def\@currentlabel{108.61}\label{stats:slow:SolveDeepDup:Unshared:time}108.61}&
 {\def\@currentlabel{2}\label{stats:slow:SolveDeepDup:Shared:mem}2} &
 {\def\@currentlabel{108.71}\label{stats:slow:SolveDeepDup:Shared:time}108.71}&
 {\def\@currentlabel{2}\label{stats:slow:SolveDeepDup:SharedThunk:mem}2} &
 {\def\@currentlabel{107.10}\label{stats:slow:SolveDeepDup:SharedThunk:time}107.10}&
 {\def\@currentlabel{2}\label{stats:slow:SolveDeepDup:SharedEvaled:mem}2} &
 {\def\@currentlabel{108.71}\label{stats:slow:SolveDeepDup:SharedEvaled:time}108.71}&
 {\def\@currentlabel{1\,641}\label{stats:slow:SolveDeepDup:SharedFull:mem}1\,641} &
 {\def\@currentlabel{118.66}\label{stats:slow:SolveDeepDup:SharedFull:time}118.66}&
 {\def\@currentlabel{2}\label{stats:slow:SolveDeepDup:RunTwice:mem}2} &
 {\def\@currentlabel{217.74}\label{stats:slow:SolveDeepDup:RunTwice:time}217.74} \\
unit lifting%
&
 {\def\@currentlabel{2}\label{stats:slow:Unit:Unshared:mem}2} &
 {\def\@currentlabel{141.49}\label{stats:slow:Unit:Unshared:time}141.49}&
 {\def\@currentlabel{2}\label{stats:slow:Unit:Shared:mem}2} &
 {\def\@currentlabel{141.48}\label{stats:slow:Unit:Shared:time}141.48}&
 {\def\@currentlabel{2}\label{stats:slow:Unit:SharedThunk:mem}2} &
 {\def\@currentlabel{141.49}\label{stats:slow:Unit:SharedThunk:time}141.49}&
&
&
&
&
 {\def\@currentlabel{2}\label{stats:slow:Unit:RunTwice:mem}2} &
 {\def\@currentlabel{282.86}\label{stats:slow:Unit:RunTwice:time}282.86} \\
church encoding%
&
 {\def\@currentlabel{2}\label{stats:slow:Church:Unshared:mem}2} &
 {\def\@currentlabel{113.23}\label{stats:slow:Church:Unshared:time}113.23}&
 {\def\@currentlabel{2}\label{stats:slow:Church:Shared:mem}2} &
 {\def\@currentlabel{113.10}\label{stats:slow:Church:Shared:time}113.10}&
 {\def\@currentlabel{2}\label{stats:slow:Church:SharedThunk:mem}2} &
 {\def\@currentlabel{113.04}\label{stats:slow:Church:SharedThunk:time}113.04}&
&
&
&
&
 {\def\@currentlabel{2}\label{stats:slow:Church:RunTwice:mem}2} &
 {\def\@currentlabel{225.74}\label{stats:slow:Church:RunTwice:time}225.74} \\
\end{tabular}
\makeatother


==> statstable.tex <==
\makeatletter
\begin{tabular}{lrrrrrrrrrrrr}
 \\
& \multicolumn{2}{c}{no sharing}& \multicolumn{2}{c}{shared tree}& \multicolumn{2}{c}{add. thunk}& \multicolumn{2}{c}{partly eval'ed}& \multicolumn{2}{c}{fully eval'ed}& \multicolumn{2}{c}{run twice} \\
& MB & sec.& MB & sec.& MB & sec.& MB & sec.& MB & sec.& MB & sec. \\ \midrule 
original%
&
 {\def\@currentlabel{2}\label{stats:Original:Unshared:mem}2} &
 {\def\@currentlabel{6.70}\label{stats:Original:Unshared:time}6.70}&
 {\def\@currentlabel{4\,189}\label{stats:Original:Shared:mem}4\,189} &
 {\def\@currentlabel{24.15}\label{stats:Original:Shared:time}24.15}&
 {\def\@currentlabel{4\,188}\label{stats:Original:SharedThunk:mem}4\,188} &
 {\def\@currentlabel{24.35}\label{stats:Original:SharedThunk:time}24.35}&
 {\def\@currentlabel{4\,188}\label{stats:Original:SharedEvaled:mem}4\,188} &
 {\def\@currentlabel{24.08}\label{stats:Original:SharedEvaled:time}24.08}&
 {\def\@currentlabel{4\,189}\label{stats:Original:SharedFull:mem}4\,189} &
 {\def\@currentlabel{30.36}\label{stats:Original:SharedFull:time}30.36}&
 {\def\@currentlabel{4\,189}\label{stats:Original:RunTwice:mem}4\,189} &
 {\def\@currentlabel{29.73}\label{stats:Original:RunTwice:time}29.73} \\
\textsf{solveDup}%
&
 {\def\@currentlabel{2}\label{stats:SolveDup:Unshared:mem}2} &
 {\def\@currentlabel{6.71}\label{stats:SolveDup:Unshared:time}6.71}&
 {\def\@currentlabel{3}\label{stats:SolveDup:Shared:mem}3} &
 {\def\@currentlabel{6.74}\label{stats:SolveDup:Shared:time}6.74}&
 {\def\@currentlabel{4\,188}\label{stats:SolveDup:SharedThunk:mem}4\,188} &
 {\def\@currentlabel{24.32}\label{stats:SolveDup:SharedThunk:time}24.32}&
 {\def\@currentlabel{4\,188}\label{stats:SolveDup:SharedEvaled:mem}4\,188} &
 {\def\@currentlabel{24.03}\label{stats:SolveDup:SharedEvaled:time}24.03}&
 {\def\@currentlabel{4\,189}\label{stats:SolveDup:SharedFull:mem}4\,189} &
 {\def\@currentlabel{30.50}\label{stats:SolveDup:SharedFull:time}30.50}&
 {\def\@currentlabel{2}\label{stats:SolveDup:RunTwice:mem}2} &
 {\def\@currentlabel{13.47}\label{stats:SolveDup:RunTwice:time}13.47} \\
\textsf{rateDup}%
&
 {\def\@currentlabel{2}\label{stats:RateDup:Unshared:mem}2} &
 {\def\@currentlabel{2.33}\label{stats:RateDup:Unshared:time}2.33}&
 {\def\@currentlabel{5}\label{stats:RateDup:Shared:mem}5} &
 {\def\@currentlabel{2.34}\label{stats:RateDup:Shared:time}2.34}&
 {\def\@currentlabel{5}\label{stats:RateDup:SharedThunk:mem}5} &
 {\def\@currentlabel{2.34}\label{stats:RateDup:SharedThunk:time}2.34}&
 {\def\@currentlabel{5}\label{stats:RateDup:SharedEvaled:mem}5} &
 {\def\@currentlabel{2.33}\label{stats:RateDup:SharedEvaled:time}2.33}&
 {\def\@currentlabel{4\,189}\label{stats:RateDup:SharedFull:mem}4\,189} &
 {\def\@currentlabel{31.28}\label{stats:RateDup:SharedFull:time}31.28}&
 {\def\@currentlabel{4\,153}\label{stats:RateDup:RunTwice:mem}4\,153} &
 {\def\@currentlabel{29.01}\label{stats:RateDup:RunTwice:time}29.01} \\
\textsf{solveDeepDup}%
&
 {\def\@currentlabel{2}\label{stats:SolveDeepDup:Unshared:mem}2} &
 {\def\@currentlabel{6.63}\label{stats:SolveDeepDup:Unshared:time}6.63}&
 {\def\@currentlabel{2}\label{stats:SolveDeepDup:Shared:mem}2} &
 {\def\@currentlabel{6.74}\label{stats:SolveDeepDup:Shared:time}6.74}&
 {\def\@currentlabel{2}\label{stats:SolveDeepDup:SharedThunk:mem}2} &
 {\def\@currentlabel{6.60}\label{stats:SolveDeepDup:SharedThunk:time}6.60}&
 {\def\@currentlabel{2}\label{stats:SolveDeepDup:SharedEvaled:mem}2} &
 {\def\@currentlabel{6.79}\label{stats:SolveDeepDup:SharedEvaled:time}6.79}&
 {\def\@currentlabel{4\,189}\label{stats:SolveDeepDup:SharedFull:mem}4\,189} &
 {\def\@currentlabel{29.72}\label{stats:SolveDeepDup:SharedFull:time}29.72}&
 {\def\@currentlabel{2}\label{stats:SolveDeepDup:RunTwice:mem}2} &
 {\def\@currentlabel{13.30}\label{stats:SolveDeepDup:RunTwice:time}13.30} \\
unit lifting%
&
 {\def\@currentlabel{1}\label{stats:Unit:Unshared:mem}1} &
 {\def\@currentlabel{1.79}\label{stats:Unit:Unshared:time}1.79}&
 {\def\@currentlabel{1}\label{stats:Unit:Shared:mem}1} &
 {\def\@currentlabel{1.78}\label{stats:Unit:Shared:time}1.78}&
 {\def\@currentlabel{1}\label{stats:Unit:SharedThunk:mem}1} &
 {\def\@currentlabel{1.78}\label{stats:Unit:SharedThunk:time}1.78}&
&
&
&
&
 {\def\@currentlabel{1}\label{stats:Unit:RunTwice:mem}1} &
 {\def\@currentlabel{3.56}\label{stats:Unit:RunTwice:time}3.56} \\
church encoding%
&
 {\def\@currentlabel{2}\label{stats:Church:Unshared:mem}2} &
 {\def\@currentlabel{7.12}\label{stats:Church:Unshared:time}7.12}&
 {\def\@currentlabel{2}\label{stats:Church:Shared:mem}2} &
 {\def\@currentlabel{7.06}\label{stats:Church:Shared:time}7.06}&
 {\def\@currentlabel{2}\label{stats:Church:SharedThunk:mem}2} &
 {\def\@currentlabel{7.19}\label{stats:Church:SharedThunk:time}7.19}&
&
&
&
&
 {\def\@currentlabel{2}\label{stats:Church:RunTwice:mem}2} &
 {\def\@currentlabel{14.35}\label{stats:Church:RunTwice:time}14.35} \\
\end{tabular}
\makeatother

